TK-Planes: Tiered K-Planes with High Dimensional Feature Vectors for Dynamic UAV-based Scenes

In this paper, we present a new approach to bridge the domain gap between synthetic and real-world data for unmanned aerial vehicle (UAV)-based perception. Our formulation is designed for dynamic scenes, consisting of small moving objects or human actions. We propose an extension of K-Planes Neural Radiance Field (NeRF), wherein our algorithm stores a set of tiered feature vectors. The tiered feature vectors are generated to effectively model conceptual information about a scene as well as an image decoder that transforms output feature maps into RGB images. Our technique leverages the information amongst both static and dynamic objects within a scene and is able to capture salient scene attributes of high altitude videos. We evaluate its performance on challenging datasets, including Okutama Action and UG2, and observe considerable improvement in accuracy over state of the art neural rendering methods.

==> Intro.tex <==
Synthetic data has been used for over a decade to train deep learning algorithms in a variety of tasks, from game play [cite old google Atari paper] to driving [cite cityscapes?].  Said data from sources such as game engines [cite unity or other source] and deep learning [cite NerF, GAN, Diffusion] have made large strides in recent years with respect to fidelity and bridging the domain gap between synthetic and real data [cite ICRA paper and Heesung paper].  Generative algorithms for instance can create realistic novel imagery and videos from a given prompt [cite], requiring an implicit model of real world objects and their codependencies.  Neural Radiance Fields and more recently Gaussian Splatting have shown impressive abilities to render both specific 3D static and dynamic scenes [cite], offering novel views of a scene not available during training.  Because of these advances, synthetic data have been playing a larger role in supplementing existing real world datasets for training data hungry perception algorithms [yolo, other percep algs].

Particular domains, such as high altitude videos from UAVs  \cite{barekatain2017okutama,}[cite UAVhuman, Okayama, others], can offer unique challenges due to the environmental conditions as well as a comparative lack of datasets under said domains.  In regard to UAVs, perception is not limited to static tasks such as object detection within a single frame but can also include more complex tasks like action recognition which can require multiple frames of a dynamic agent.  The inclusion of dynamic objects and agents further compounds the difficulty of a task and accentuates the need for large amounts of data.  Esoteric tasks, for example search and rescue, add another layer of complication as more general datasets may not capture the requisite environmental detail and conditions or relevant agent behavior.

Given a dynamic UAV scene, several issues become pertinent when trying to model accurate dynamic behavior.  First, because of the nature of high altitude data, target objects are often at a large distance from the camera and appear small relative to the background.  Due to the more difficult task of modeling dynamic objects, this imbalance between static and dynamic elements of a scene can cause issues with separating static and dynamic elements within any given algorithm, in particular if there are inaccuracies present in camera pose information.  Second, dynamic objects are often sparse in the scene at any given point of time.  This further limits the amount of data that can afford training.  Lastly, diverse poses at specific time stamps may be limited, often with just one camera pose per timestamp and limited variation in camera poses.  This can lead to degeneracies in the output of a model the more poses and their corresponding timestamps diverge from the training data.

\noindent {\bf Main Results:} Our method aims to rectify these issues with a novel Neural Radiance Field architecture.   We have developed a tiered version of the K-Planes algorithm, TK-Planes, that outputs and operates on feature vectors rather than RGB pixel values.  These feature vectors can store conceptual information about a particular object or location within a scene and  when output for multiple corresponding camera rays, form feature maps that are decoded to form a final image.  Furthermore, taking advantage of the fact that many details of a scene, including dynamic objects, repeat throughout, sets of feature vectors for static and dynamic elements are shared amongst grid cells in the TK-Planes algorithm.  Sharing these vectors means that the algorithm can learn how to model dynamic objects for instance from the mutual information of all dynamic objects within the scene, rather than independently for each one.
